Morality is Non-Binary: Building a Pluralist Moral Sentence Embedding Space using Contrastive Learning

Recent advances in NLP show that language models retain a discernible level of knowledge in deontological ethics and moral norms. However, existing works often treat morality as binary, ranging from right to wrong. This simplistic view does not capture the nuances of moral judgment. Pluralist moral philosophers argue that human morality can be deconstructed into a finite number of elements, respecting individual differences in moral judgment. In line with this view, we build a pluralist moral sentence embedding space via a state-of-the-art contrastive learning approach. We systematically investigate the embedding space by studying the emergence of relationships among moral elements, both quantitatively and qualitatively. Our results show that a pluralist approach to morality can be captured in an embedding space. However, moral pluralism is challenging to deduce via self-supervision alone and requires a supervised approach with human labels.

==> sections_resubmission/app-table.tex <==

\begin{table*}[!htb]
\centering
\scriptsize
\begin{subtable}{0.49\linewidth}
\centering
\scriptsize
\renewcommand{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{rccccc|ccccc}
 & \rot{\textbf{Care}} & \rot{\textbf{Fairness}} & \rot{\textbf{Loyalty}} & \rot{\textbf{Authority}} & \rot{\textbf{Purity}} & \rot{\textbf{Harm}} & \rot{\textbf{Cheating}} & \rot{\textbf{Betrayal}} & \rot{\textbf{Subversion}} & \rot{\textbf{Degradation}} \\
\textbf{Care} & {\cellcolor[HTML]{2081B9}} \color[HTML]{F1F1F1} 45.3 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.7 & {\cellcolor[HTML]{81AED2}} \color[HTML]{F1F1F1} 37.0 & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} 34.9 & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} 35.2 & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.8 & {\cellcolor[HTML]{DEDCEC}} \color[HTML]{000000} 26.3 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.8 & {\cellcolor[HTML]{C9CEE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} 24.2 \\
\textbf{Fairness} & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.7 & {\cellcolor[HTML]{569DC8}} \color[HTML]{F1F1F1} 40.7 & {\cellcolor[HTML]{A9BFDC}} \color[HTML]{000000} 33.1 & {\cellcolor[HTML]{83AFD3}} \color[HTML]{F1F1F1} 36.9 & {\cellcolor[HTML]{96B6D7}} \color[HTML]{000000} 35.1 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.3 & {\cellcolor[HTML]{71A8CE}} \color[HTML]{F1F1F1} 38.6 & {\cellcolor[HTML]{9EBAD9}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{96B6D7}} \color[HTML]{000000} 35.0 & {\cellcolor[HTML]{AFC1DD}} \color[HTML]{000000} 32.5 \\
\textbf{Loyalty} & {\cellcolor[HTML]{81AED2}} \color[HTML]{F1F1F1} 37.0 & {\cellcolor[HTML]{A9BFDC}} \color[HTML]{000000} 33.1 & {\cellcolor[HTML]{2786BB}} \color[HTML]{F1F1F1} 44.7 & {\cellcolor[HTML]{71A8CE}} \color[HTML]{F1F1F1} 38.5 & {\cellcolor[HTML]{80AED2}} \color[HTML]{F1F1F1} 37.2 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{B4C4DF}} \color[HTML]{000000} 31.9 & {\cellcolor[HTML]{ADC1DD}} \color[HTML]{000000} 32.6 & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} 35.0 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 \\
\textbf{Authority} & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} 34.9 & {\cellcolor[HTML]{83AFD3}} \color[HTML]{F1F1F1} 36.9 & {\cellcolor[HTML]{71A8CE}} \color[HTML]{F1F1F1} 38.5 & {\cellcolor[HTML]{4A98C5}} \color[HTML]{F1F1F1} 41.6 & {\cellcolor[HTML]{67A4CC}} \color[HTML]{F1F1F1} 39.4 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 30.6 & {\cellcolor[HTML]{9FBAD9}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} 32.8 & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} 36.0 & {\cellcolor[HTML]{B0C2DE}} \color[HTML]{000000} 32.3 \\
\textbf{Purity} & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} 35.2 & {\cellcolor[HTML]{96B6D7}} \color[HTML]{000000} 35.1 & {\cellcolor[HTML]{80AED2}} \color[HTML]{F1F1F1} 37.2 & {\cellcolor[HTML]{67A4CC}} \color[HTML]{F1F1F1} 39.4 & {\cellcolor[HTML]{157AB5}} \color[HTML]{F1F1F1} 46.4 & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} 32.8 & {\cellcolor[HTML]{9CB9D9}} \color[HTML]{000000} 34.4 & {\cellcolor[HTML]{9CB9D9}} \color[HTML]{000000} 34.4 & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} 36.0 & {\cellcolor[HTML]{5EA0CA}} \color[HTML]{F1F1F1} 40.1 \\
\hhline{~----------}
\textbf{Harm} & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.8 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.3 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 30.6 & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} 32.8 & {\cellcolor[HTML]{1077B4}} \color[HTML]{F1F1F1} 46.9 & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} 35.2 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 & {\cellcolor[HTML]{79ABD0}} \color[HTML]{F1F1F1} 37.8 & {\cellcolor[HTML]{589EC8}} \color[HTML]{F1F1F1} 40.5 \\
\textbf{Cheating} & {\cellcolor[HTML]{DEDCEC}} \color[HTML]{000000} 26.3 & {\cellcolor[HTML]{71A8CE}} \color[HTML]{F1F1F1} 38.6 & {\cellcolor[HTML]{B4C4DF}} \color[HTML]{000000} 31.9 & {\cellcolor[HTML]{9FBAD9}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{9CB9D9}} \color[HTML]{000000} 34.4 & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} 35.2 & {\cellcolor[HTML]{3D93C2}} \color[HTML]{F1F1F1} 42.6 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 & {\cellcolor[HTML]{76AAD0}} \color[HTML]{F1F1F1} 38.1 & {\cellcolor[HTML]{69A5CC}} \color[HTML]{F1F1F1} 39.2 \\
\textbf{Betrayal} & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.8 & {\cellcolor[HTML]{9EBAD9}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{ADC1DD}} \color[HTML]{000000} 32.6 & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} 32.8 & {\cellcolor[HTML]{9CB9D9}} \color[HTML]{000000} 34.4 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 & {\cellcolor[HTML]{3790C0}} \color[HTML]{F1F1F1} 43.1 & {\cellcolor[HTML]{4C99C5}} \color[HTML]{F1F1F1} 41.5 & {\cellcolor[HTML]{4496C3}} \color[HTML]{F1F1F1} 42.0 \\
\textbf{Subversion} & {\cellcolor[HTML]{C9CEE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{96B6D7}} \color[HTML]{000000} 35.0 & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} 35.0 & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} 36.0 & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} 36.0 & {\cellcolor[HTML]{79ABD0}} \color[HTML]{F1F1F1} 37.8 & {\cellcolor[HTML]{76AAD0}} \color[HTML]{F1F1F1} 38.1 & {\cellcolor[HTML]{4C99C5}} \color[HTML]{F1F1F1} 41.5 & {\cellcolor[HTML]{2C89BD}} \color[HTML]{F1F1F1} 44.2 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 \\
\textbf{Degradation} & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} 24.2 & {\cellcolor[HTML]{AFC1DD}} \color[HTML]{000000} 32.5 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{B0C2DE}} \color[HTML]{000000} 32.3 & {\cellcolor[HTML]{5EA0CA}} \color[HTML]{F1F1F1} 40.1 & {\cellcolor[HTML]{589EC8}} \color[HTML]{F1F1F1} 40.5 & {\cellcolor[HTML]{69A5CC}} \color[HTML]{F1F1F1} 39.2 & {\cellcolor[HTML]{4496C3}} \color[HTML]{F1F1F1} 42.0 & {\cellcolor[HTML]{63A2CB}} \color[HTML]{F1F1F1} 39.6 & {\cellcolor[HTML]{045F95}} \color[HTML]{F1F1F1} 51.7 \\
\end{tabular}
\caption{Moral similarity of MoralStrength (supervised SimCSE).}
\label{tab:moral-sim-strength}
%\end{minipage}%
\end{subtable}
\hfill
\begin{subtable}{0.49\linewidth}
\centering
\scriptsize
\renewcommand{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{rccccc|ccccc}
 & \rot{\textbf{Care}} & \rot{\textbf{Fairness}} & \rot{\textbf{Loyalty}} & \rot{\textbf{Authority}} & \rot{\textbf{Purity}} & \rot{\textbf{Harm}} & \rot{\textbf{Cheating}} & \rot{\textbf{Betrayal}} & \rot{\textbf{Subversion}} & \rot{\textbf{Degradation}} \\
\textbf{Care} & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} 32.9 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 28.0 & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 27.9 & {\cellcolor[HTML]{CACEE5}} \color[HTML]{000000} 29.3 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.3 \\
\textbf{Fairness} & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 28.0 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 30.6 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.7 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 28.3 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.8 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 27.6 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.9 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 28.7 & {\cellcolor[HTML]{CACEE5}} \color[HTML]{000000} 29.3 & {\cellcolor[HTML]{D3D4E7}} \color[HTML]{000000} 28.1 \\
\textbf{Loyalty} & {\cellcolor[HTML]{C6CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.7 & {\cellcolor[HTML]{B3C3DE}} \color[HTML]{000000} 32.0 & {\cellcolor[HTML]{C9CEE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.2 & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.3 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{C4CBE3}} \color[HTML]{000000} 30.0 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 28.0 \\
\textbf{Authority} & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 28.3 & {\cellcolor[HTML]{C9CEE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{BCC7E1}} \color[HTML]{000000} 30.9 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 28.7 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.3 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 \\
\textbf{Purity} & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 27.8 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{B8C6E0}} \color[HTML]{000000} 31.4 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 28.4 & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.7 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.6 \\
\hhline{~----------}
\textbf{Harm} & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 27.6 & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.2 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} 33.3 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{BDC8E1}} \color[HTML]{000000} 30.8 & {\cellcolor[HTML]{B7C5DF}} \color[HTML]{000000} 31.5 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.9 \\
\textbf{Cheating} & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 27.9 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.9 & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.3 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 28.7 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 28.4 & {\cellcolor[HTML]{CDD0E5}} \color[HTML]{000000} 29.0 & {\cellcolor[HTML]{B0C2DE}} \color[HTML]{000000} 32.3 & {\cellcolor[HTML]{C4CBE3}} \color[HTML]{000000} 30.0 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 30.6 & {\cellcolor[HTML]{CCCFE5}} \color[HTML]{000000} 29.2 \\
\textbf{Betrayal} & {\cellcolor[HTML]{CACEE5}} \color[HTML]{000000} 29.3 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 28.7 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.8 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{CED0E6}} \color[HTML]{000000} 28.9 & {\cellcolor[HTML]{BDC8E1}} \color[HTML]{000000} 30.8 & {\cellcolor[HTML]{C4CBE3}} \color[HTML]{000000} 30.0 & {\cellcolor[HTML]{B0C2DE}} \color[HTML]{000000} 32.4 & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} 32.2 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.2 \\
\textbf{Subversion} & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.5 & {\cellcolor[HTML]{CACEE5}} \color[HTML]{000000} 29.3 & {\cellcolor[HTML]{C4CBE3}} \color[HTML]{000000} 30.0 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.3 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.7 & {\cellcolor[HTML]{B7C5DF}} \color[HTML]{000000} 31.5 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 30.6 & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} 32.2 & {\cellcolor[HTML]{9FBAD9}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{C0C9E2}} \color[HTML]{000000} 30.4 \\
\textbf{Degradation} & {\cellcolor[HTML]{D2D3E7}} \color[HTML]{000000} 28.3 & {\cellcolor[HTML]{D3D4E7}} \color[HTML]{000000} 28.1 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 28.0 & {\cellcolor[HTML]{D1D2E6}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 29.6 & {\cellcolor[HTML]{C5CCE3}} \color[HTML]{000000} 29.9 & {\cellcolor[HTML]{CCCFE5}} \color[HTML]{000000} 29.2 & {\cellcolor[HTML]{C2CBE2}} \color[HTML]{000000} 30.2 & {\cellcolor[HTML]{C0C9E2}} \color[HTML]{000000} 30.4 & {\cellcolor[HTML]{B8C6E0}} \color[HTML]{000000} 31.5 \\
\end{tabular}
\caption{Moral Similarity of MoralStrength (unsupervised SimCSE).}
\label{tab:moral-sim-strength-unsup}
%\end{minipage}%
\end{subtable}
    \caption{Moral Similarity tables of MFD2.0 and MoralStrength with supervised and unsupervised SimCSE.}
    \label{tab:moral-similarity-moralStrength}
\end{table*}

